Bayesian Generational Population-Based Training

Reinforcement learning (RL) offers the potential for training generally capable agents that can interact autonomously in the real world. However, one key limitation is the brittleness of RL algorithms to core hyperparameters and network architecture choice. Furthermore, non-stationarities such as evolving training data and increased agent complexity mean that different hyperparameters and architectures may be optimal at different points of training. This motivates AutoRL, a class of methods seeking to automate these design choices. One prominent class of AutoRL methods is Population-Based Training (PBT), which have led to impressive performance in several large scale settings. In this paper, we introduce two new innovations in PBT-style methods. First, we employ trust-region based Bayesian Optimization, enabling full coverage of the high-dimensional mixed hyperparameter search space. Second, we show that using a generational approach, we can also learn both architectures and hyperparameters jointly on-the-fly in a single training run. Leveraging the new highly parallelizable Brax physics engine, we show that these innovations lead to large performance gains, significantly outperforming the tuned baseline while learning entire configurations on the fly. Code is available at https://github.com/xingchenwan/bgpbt.

==> 09_reproducibility.tex <==
\clearpage
\section{Reproducibility Checklist}


\begin{enumerate}
\item For all authors\dots
  \begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately
    reflect the paper's contributions and scope?
    \answerYes{[The abstract and introduction's content is substantiated in §\ref{sec:experiments}]}
  \item Did you describe the limitations of your work?
    \answerYes{We discuss them in §\ref{sec:conclusion}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{We discuss them in §\ref{sec:conclusion}.}
  \item Have you read the ethics review guidelines and ensured that your paper
    conforms to them?
    \answerYes{We have ensured our paper conforms to the guidelines.}
  \end{enumerate}
\item If you are including theoretical results\dots
  \begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{The full set of assumptions are provided in \cref{app:proofs}.}
  \item Did you include complete proofs of all theoretical results?
    \answerYes{Complete proofs provided in \cref{app:proofs}.}
  \end{enumerate}
\item If you ran experiments\dots
  \begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the
    main experimental results, including all requirements (e.g.,
    \texttt{requirements.txt} with explicit version), an instructive
    \texttt{README} with installation, and execution commands (either in the
    supplemental material or as a \textsc{url})?
    \answerYes{We have included this in the supplementary material.}
  \item Did you include the raw results of running the given instructions on the
    given code and data?
    \answerYes{We include raw numbers produced by the code.}
  \item Did you include scripts and commands that can be used to generate the
    figures and tables in your paper based on the raw results of the code, data,
    and instructions given?
    \answerYes{We include notebooks that produce the plots.}
  \item Did you ensure sufficient code quality such that your code can be safely
    executed and the code is properly documented?
    \answerYes{Yes, the code is documented and appropriate commands provided.}
  \item Did you specify all the training details (e.g., data splits,
    pre-processing, search spaces, fixed hyperparameter settings, and how they
    were chosen)?
    \answerYes{Implementation details are discussed in \cref{app:full_search_space} and \cref{app:implementation_details}.}
  \item Did you ensure that you compared different methods (including your own)
    exactly on the same benchmarks, including the same datasets, search space,
    code for training and hyperparameters for that code?
    \answerYes{All methods benchmarked on the same \textsc{Brax} environment suite, we used the same computational budget and population size for all other PBT methods.}
  \item Did you run ablation studies to assess the impact of different
    components of your approach?
    \answerYes{We include ablations in \cref{sec:experiments} and in \cref{app:additional_experiments}.}
  \item Did you use the same evaluation protocol for the methods being compared?
    \answerYes{All PBT methods are evaluated by best performance in the population.}
  \item Did you compare performance over time?
    \answerYes{We regularly evaluate the evaluated performance through the course of training.}
  \item Did you perform multiple runs of your experiments and report random seeds?
    \answerYes{All our experiments are averaged over 7 random seeds.}
  \item Did you report error bars (e.g., with respect to the random seed after
    running experiments multiple times)?
    \answerYes{We report the mean performance and indicate $\pm$ 1 standard error.}
  \item Did you use tabular or surrogate benchmarks for in-depth evaluations?
    \answerNA{}{}
  \item Did you include the total amount of compute and the type of resources
    used (e.g., type of \textsc{gpu}s, internal cluster, or cloud provider)?
    \answerYes{We describe our compute and resource usage in \cref{app:implementation_details}.}
  \item Did you report how you tuned hyperparameters, and what time and
    resources this required (if they were not automatically tuned by your AutoML method, e.g. in a \textsc{nas} approach; and also hyperparameters of your
    own method)?
    \answerYes{The RL hyperparameters were tuned by our AutoRL method. The hyperparameters for \our were tuned by hand with ablations performed in \cref{app:additional_experiments}.}
  \end{enumerate}
\item If you are using existing assets (e.g., code, data, models) or
  curating/releasing new assets\dots
  \begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We cite the creators of the codebase we use in \cref{app:implementation_details}.}
  \item Did you mention the license of the assets?
    \answerYes{We mention the license of the codebase we use in \cref{app:implementation_details}.}
  \item Did you include any new assets either in the supplemental material or as a \textsc{url}?
    \answerYes{We include figures in a url link in the introduction.}
  \item Did you discuss whether and how consent was obtained from people whose
    data you're using/curating?
    \answerNA{No personal data used. All data for our algorithm is generated from RL environments.}
  \item Did you discuss whether the data you are using/curating contains
    personally identifiable information or offensive content?
    \answerNA{No personal data used. All data for our algorithm is generated from RL environments.}
  \end{enumerate}
\item If you used crowdsourcing or conducted research with human subjects\dots
  \begin{enumerate}
  \item Did you include the full text of instructions given to participants and
    screenshots, if applicable?
    \answerNA{[We are not crowdsourcing or conducting research with human subjects.]}
  \item Did you describe any potential participant risks, with links to
    Institutional Review Board (\textsc{irb}) approvals, if applicable?
    \answerNA{[We are not crowdsourcing or conducting research with human subjects.]}
  \item Did you include the estimated hourly wage paid to participants and the
    total amount spent on participant compensation?
    \answerNA{[We are not crowdsourcing or conducting research with human subjects.]}
  \end{enumerate}
\end{enumerate}

==> BG-PBT (AutoML Conference)_arXiv 2/01_abstract.tex <==
\begin{abstract}
Reinforcement learning (RL) offers the potential for training generally capable agents that can interact autonomously in the real world.
However, one key limitation is the brittleness of RL algorithms to core hyperparameters and network architecture choice.
Furthermore, non-stationarities such as evolving training data and increased agent complexity mean that different hyperparameters and architectures may be optimal at different points of training.
This motivates AutoRL, a class of methods seeking to automate these design choices.
One prominent class of AutoRL methods is Population-Based Training (PBT), which have led to impressive performance in several large scale settings.
In this paper, we introduce two new innovations in PBT-style methods.
First, we employ trust-region based Bayesian Optimization, enabling full coverage of the high-dimensional mixed hyperparameter search space.
Second, we show that using a \emph{generational} approach, we can also learn both architectures and hyperparameters jointly on-the-fly in a single training run.
Leveraging the new highly parallelizable Brax physics engine, we show that these innovations lead to large performance gains, significantly outperforming the tuned baseline while learning entire configurations on the fly. Code is available at \url{https://github.com/xingchenwan/bgpbt}.
\end{abstract}




==> BG-PBT (AutoML Conference)_arXiv 2/02_intro.tex <==
\section{Introduction}
\gls{RL} \citep{Sutton1998} has proven to be a successful paradigm for training agents across a variety of domains and tasks~\citep{mnih-atari-2013, alphago, qtopt, nguyen2021deep}, with some believing it could be enough for training generally capable agents~\citep{rewardenough}.
However, a crucial factor limiting the wider applicability of \gls{RL} to new problems is the notorious sensitivity of algorithms with respect to their hyperparameters~\citep{deeprlmatters, andrychowicz2021what, Engstrom2020Implementation}, which often require expensive tuning.
Indeed, it has been shown that when tuned effectively, good configurations often lead to dramatically improved performance in large scale settings~\citep{bo_alphago}.

To address these challenges, recent work in \emph{Automated Reinforcement Learning} (AutoRL) \citep{autorl_survey} has shown that rigorously searching these parameter spaces can lead to previously unseen levels of performance, even capable of breaking widely used simulators~\citep{pbtbt}.
However, {AutoRL} contains unique challenges, as different tasks even in the same suite are often best solved with different network architectures and hyperparameters~\citep{furuta2021pic, xu2022accelerated}.
Furthermore, due to the non-stationarities present in \gls{RL}~\citep{igl2021transient}, such as changing data distributions and the requirement for agents to model increasingly complex behaviors over time, optimal hyperparameters and architectures may not remain constant.
To address this, works have shown adapting hyperparameters through time~\citep{paul2019fast, pbtbt, parkerholder2021tuning, PBT} and defining fixed network architecture schedules~\citep{czarnecki2018mixmatch} can be beneficial for performance.
However, architectures and hyperparameters are inherently linked~\citep{networkwidthlearningrate}, and to date, no method combines the ability to jointly and continuously adapt both on the fly.

In this paper we focus on \gls{PBT} \citep{PBT} methods, where a population of agents is trained in parallel, copying across stronger weights and enabling adaption of hyperparameters in a single training run.
This allows \gls{PBT} methods to achieve impressive performance on many large-scale settings~\citep{capturetheflag, pbtfootball}.
However, \gls{PBT}-style methods are typically limited in scope due to two key factors: 1) they only optimize a handful of hyperparameters, either due to using random search \citep{PBT}, or model-based methods that do not scale to higher dimensions~\citep{pb2, parkerholder2021tuning};
2) \gls{PBT} methods are usually restricted to the same fixed architecture since weights are copied between agents.

\begin{figure}[t]
    \begin{center}
        \includegraphics[trim=0cm 0cm 0cm  -1.1cm, clip, width=1.0\linewidth]{figures/cover_fig.pdf}   
    \end{center}
    \vspace{-5mm}
        \caption{An example run of \textsc{bg-pbt} on HalfCheetah task in \textsc{Brax}: \textsc{bg-pbt} combines population-based training with high-dimensional Bayesian optimization, generational training (different generations marked with numbers in the figure) and on-policy distillation between generations to transfer across \gls{RL} agents with different neural architectures: at different points during training, both hyperparameters and the architectures of policy \& value networks are tuned on-the-fly, leading to significant improvement over the baseline.
        }
        \label{fig:cover_fig}
        \vspace{-8mm}
\end{figure}

We seek to overcome both of these issues in this paper, and propose \emph{\ourNAS}, with an example run demonstrated in Fig.~\ref{fig:cover_fig}.
\ourNAS is capable of tuning a significantly greater proportion of the agent's configuration, thanks to two new ideas.
First, we introduce a new model-based \emph{hyperparameter and architecture} exploration step motivated by recent advances in local Bayesian optimization~\citep{casmopolitan}.
Second, we take inspiration from \citet{openendedlearningteam2021openended} who showed that \gls{PBT} can be particularly effective when combined with network distillation~\citep{igl2021transient}, in an approach known as generational learning.
As prior works in generational training~\citep{alphastar, openendedlearningteam2021openended} show, the use of successive generations of architectures with distillation results in significantly reduced training time for new agents.
This provides us with an algorithm-agnostic framework to create agents which continuously discover their \emph{entire configuration}.
Thus, for the first time, we can tune hyperparameters and architectures during one training run as part of a single unified algorithm.

We run a series of exhaustive experiments tuning both the architectures and hyperparameters for a \gls{PPO}~\citep{ppo}  agent in the newly introduced \textsc{Brax} environment suite~\citep{brax}.
\textsc{Brax} enables massively parallel simulation of agents, making it perfect for testing population-based methods without vast computational resources.
Our agents significantly outperform both the tuned baseline and a series of prior \gls{PBT} methods.
Notably, we observe that \ourNAS often discovers a \emph{schedule of networks} during training---which would be infeasible to train from scratch.
Furthermore, \ourNAS discovers entirely new modes of behavior for these representative environments, which we show at \url{https://sites.google.com/view/bgpbt}. 

To summarize, the main contributions of this paper are as follows:
\begin{enumerate}[noitemsep,topsep=-8pt, leftmargin=3pt]
    \item We show for the first time it is possible to select architectures as part of a \textcolor{blue}{general-purpose} \gls{PBT} framework, using \textit{generational training with policy distillation} with \gls{NAS}.
    \item We propose a novel and efficient algorithm, \textbf{\ourNAS}, especially designed for high-dimensional mixed search spaces, which can select both architectures and hyperparameters on-the-fly with provable efficiency guarantees.
    \item We show in a series of experiments our \textit{automatic architecture curricula} make it possible to achieve significantly higher performance than previous methods.
\end{enumerate}


==> BG-PBT (AutoML Conference)_arXiv 2/03_background.tex <==
\section{Preliminaries}
We begin by introducing the reinforcement learning framework, population-based training, which our method is based on, and the general problem setup we investigate in this paper.

\textbf{Reinforcement Learning.}
We model the environment as a \gls{MDP} \citep{Sutton1998}, defined as a tuple $M = (\mathcal{S}, \mathcal{A}, P, R, \rho_0, \gamma)$, where $\mathcal{S}$ and $\mathcal{A}$ denote the state and action spaces respectively, $P(s_{t+1} | s_t, a_t)$  the transition dynamics, $R(s_t, a_t)$  the reward function, $ \rho_0$  the initial state distribution, and $\gamma \in (0, 1)$ the discount factor.
The goal is to optimize a policy $\pi (a_t | s_t)$ that maximizes the expected discounted return $\mathbb{E}_{\pi, P, \rho_0}\left[\sum_{t=0}^\infty \gamma^t R(s_t, a_t)\right]$.
Given a policy $\pi$, we may define the state value function $V^{\pi}(s) = \mathbb{E}_{\pi, P}\left[\sum_{t=0}^\infty \gamma^t R(s_t, a_t) | s_0 = s \right]$ and the state-action value-function $Q^{\pi}(s, a) = \mathbb{E}_{\pi, P}\left[\sum_{t=0}^\infty \gamma^t R(s_t, a_t) | s_0 = s, a_0 = a \right]$. The advantage function is then defined as the difference $A^{\pi}(s, a) = Q^{\pi}(s, a) - V^{\pi}(s)$.

A popular algorithm for online continuous control that we use is \gls{PPO} \citep{ppo}.
\gls{PPO} achieves state-of-the-art results for popular benchmarks~\citep{procgen} and is hugely parallelizable, making it an ideal candidate for population-based methods~\citep{pb2}.
\gls{PPO} approximates \textsc{trpo} ~\citep{ppo, trpo} and uses a clipped objective to stabilize training:
\begin{align}
\label{eqn:ppo}
\mathcal{L}_{\mathrm{PPO}}(\theta)=\min \left(\frac{\pi_{\theta}(a \mid s)}{\pi_{\mu}(a \mid s)} A^{\pi_{\mu}}, g(\theta, \mu) A^{\pi_{\mu}}\right), \text { where } g(\theta, \mu)=\operatorname{clip}\left(\frac{\pi_{\theta}(a \mid s)}{\pi_{\mu}(a \mid s)}, 1-\epsilon, 1+\epsilon\right)
\end{align}
where $\pi_{\mu}$ is a previous policy and $\epsilon$ is the clipping parameter.

\textbf{Population-Based Training.}
\gls{RL} algorithms, including \gls{PPO}, are typically quite sensitive to their hyperparameters.
\gls{PBT} \citep{PBT} is an evolutionary method that tunes \gls{RL} hyperparameters on-the-fly.
It optimizes a population of $B$ agents in parallel, so that their weights and hyperparameters may be dynamically adapted within a single training run.
In the standard paradigm without architecture search, we consider two sub-routines, $\mathrm{explore}$ and $\mathrm{exploit}$.
We train for a total of $T$ steps and evaluate performance every $t_{\mathrm{ready}} < T$ steps.
In the $\mathrm{exploit}$ step, the weights of the worst-performing agents are replaced by those from an agent randomly sampled from the set of best-performing ones, via \emph{truncation selection}.
To select new hyperparameters, we perform the $\mathrm{explore}$ step.
We denote the hyperparameters for the $b$th agent in a population at timestep $t$ as $\bz_t^b\in\mathcal{Z}$;
this defines a \textit{schedule} of hyperparameters over time $\left( z_t^b \right)_{t=1,...T}$.
Let $f_t(z_t)$ be an objective function (e.g. the return of a \gls{RL} agent) under a given set of hyperparameters at timestep $t$, our goal is to maximize the final performance $f_T(z_T)$.

The original \gls{PBT} uses a combination of random sampling and evolutionary search for the explore step by suggesting new hyperparameters mutated from the best-performing agents.
\gls{PB2} and \gls{PB2}-Mix \citep{pb2, parkerholder2021tuning} improve on \gls{PBT} by using \emph{\gls{BO}} to suggest new hyperparameters, relying on a time-varying \emph{\gls{GP}} \citep{RasmussenGP, bogunovic2016time} to model the data observed.
We will also use \gls{GP}-based \gls{BO} in our method, and we include a primer of \gls{GP}s and \gls{BO} in App. \ref{app:primer}.

\textbf{Problem Setup.}
We follow the notation used in \cite{pb2} and frame the hyperparameter optimization problem in the lens of optimizing an expensive, time-varying, black-box reward function $f_t : \mathcal{Z} \rightarrow \mathbb{R}$.
Every $t_{\mathrm{ready}}$ steps, we observe and record noisy observations, $y_t = f_t(\bz_t) + \epsilon_t$, where $\epsilon_t \sim \mathcal{N}(0, \sigma^2\mathbf{I})$ for some fixed variance $\sigma^2$.
We follow the typical \gls{PBT} setup by defining a hyperparameter space, $\mathcal{Z}$, which for the \textsc{Brax}~\citep{brax} implementation of \gls{PPO} we follow in the paper, 
consists of 9 parameters: learning rate, discount factor ($\gamma$), entropy coefficient ($c$), unroll length, reward scaling, batch size, updates per epoch, GAE parameter ($\lambda$) and clipping parameter ($\epsilon$).
To incorporate the architecture hyperparameters, $\by \in \mathcal{Y}$, we add 6 additional parameters leading to a 15-dimensional joint space $\mathcal{J} = \mathcal{Y} \times \mathcal{Z}$.
For both the policy and value networks, we add the width and depth of the \gls{MLP} and a binary flag on whether to use spectral normalization.




==> BG-PBT (AutoML Conference)_arXiv 2/05_method.tex <==
\section{Bayesian Generational Population-Based Training (BG-PBT)}
\begin{wrapfigure}{R}{0.5\textwidth}
\vspace{-7.5mm}
    \begin{minipage}{0.5\textwidth}
\begin{algorithm}[H]
\begin{footnotesize}
	    \caption{\ourNAS;
	    distillation and \gls{NAS} steps marked in \textcolor{magenta}{magenta} (§\ref{subsec:distillation})
	   %
	    }
	    \label{alg:main_alg}
	\begin{algorithmic}[1]
		\STATE {\bfseries Input}: pop size $B$, $t_{\mathrm{ready}}$, max steps $T$, $q$ (\% agents replaced per iteration)
		\STATE \textbf{Initialize} $B$ agents with weights $\{\theta_0^{(i)}\}_{i=1}^B$, random hyperparameters $\{\bz_0^{(i)}\}_{i=1}^B$ \textcolor{magenta}{and architectures $\{\by_0^{(i)}\}_{i=1}^B$},  %
        \FOR{$t=1, \dots, T$ (in parallel for all $B$ agents)}
        \STATE Train models \& record data for all agents 
        \IF {$t~\mathrm{mod}~t_{\mathrm{ready}} = 0$}
            \STATE Replace the weights \textcolor{magenta}{\& architectures} of the bottom $q \%$ agents with those of the top $q \%$ agents.
            \STATE Update the surrogate with new observations \& returns and adjust/restart the trust regions.
            \STATE \textcolor{magenta}{Check whether to start a new generation (see §\ref{subsec:distillation}).}%
            \IF {\textcolor{magenta}{start a new generation}}
            \STATE \textcolor{magenta}{Clear the \gls{GP} training data.}
            \STATE \textcolor{magenta}{Create $B$ agents with archs.~from BO/random.}
            \STATE \textcolor{magenta}{Distill from a top-$q\%$ performing agent of the existing generation to new agents.}
            \ELSE \STATE{Select new hyperparameters $\bz$ for the agents whose weights have been just replaced with randomly sampled configs (if $\mathbf{D} = \emptyset$) \textbf{OR} using the suggestions from the \gls{BO} agent described \textcolor{magenta}{conditioned on $\by$} (otherwise)}.
            \ENDIF
        \ENDIF
    	\ENDFOR
	\end{algorithmic}
\end{footnotesize}
\end{algorithm}
\end{minipage}
\vspace{-9mm}
\end{wrapfigure}
We present \our in \cref{alg:main_alg} which consists of two major components. First, a \gls{BO} approach to select new hyperparameter configurations $\bz$ for our agents (§\ref{subsec:bo}).
We then extend the search space to accommodate architecture search, allowing agents to choose their own networks (parameterized by $\by \in \mathcal{Y}$) and use on-policy distillation to transfer between different architectures (§\ref{subsec:distillation}). 

\subsection{High-Dimensional BO Agents in Mixed-Input Configuration Space for PBT}
\label{subsec:bo}



Existing population-based methods ignore (\gls{PB2}) or only partially address (\gls{PB2}-Mix, which does not consider ordinal variables such as integers) the heterogeneous nature of the mixed hyperparameter space $\mathcal{Z}$.
Furthermore, both previous methods are equipped with standard \gls{GP} surrogates which typically scale poorly beyond low-dimensional search spaces, and are thus only used to tune a few selected hyperparameters deemed to be the most important based on human expertise.
To address these issues, \our explicitly accounts for the characteristics of typical \gls{RL} hyperparameter search space by making several novel extensions to \textsc{Casmopolitan} \citep{casmopolitan}, a state-of-the-art \gls{BO} method for high-dimensional, mixed-input problems for our setting.
In this section, we outline the main elements of our design, and we refer the reader to  App. \ref{appsubsec:propose} for full technical details of the approach.

\textbf{Tailored Treatment of Mixed Hyperparameter Types.}
Hyperparameters in \gls{RL} can be continuous (e.g. discounting factor), ordinal (discrete variables with ordering, e.g. batch size) and categorical (discrete variables without ordering, e.g. activation function).
\our treats each variable type differently: we use tailored kernels for the \gls{GP} surrogate, and utilize interleaved optimization for the acquisition function, alternating between local search for the categorical/ordinal variables and gradient descent for the continuous variables.
\our extends both \textsc{Casmopolitan} and \gls{PB2}-Mix by further accommodating ordinal variables, as both previous works only considered continuous and categorical variables.
We demonstrate the considerable benefits of explicitly accounting for the ordinal variables in App. \ref{app:ablation_ordinal}.


\textbf{\gls{TR}.} 
\gls{TR}s have proven success in extending \gls{GP}-based \gls{BO} to higher-dimensional search spaces, which were previously intractable due to the curse of dimensionality, by limiting exploration to promising regions in the search space based on past observations \citep{eriksson2019scalable, casmopolitan}.
In the \gls{PBT} context, \gls{TR}s also implicitly avoid large jumps in hyperparameters, which improves training stability. 
We adapt the \gls{TR}s used in the original \textsc{Casmopolitan} to the time-varying setup by defining \gls{TR}s around the current best configuration, and then adjusting them dynamically: 
similar to \citet{eriksson2019scalable} and \citet{casmopolitan}, \gls{TR}s are expanded or shrunk upon consecutive ``successes'' or ``failures''.
We define a proposed configuration to be a ``success'' if it appears in the top $q\%$-performing agents and a ``failure'' otherwise. 
When the \gls{TR}s shrink below some specified minimum, a \emph{restart} is triggered, which resets the \gls{GP} surrogate to avoid becoming stuck at a local optimum.
We adapt the \gls{UCB}-based criterion proposed in~\citet{casmopolitan} which is based on a global, auxiliary \gls{GP} model to the time-varying setting to re-initialize the population when a restart is triggered.
Full details are provided in App. \ref{appsubsec:restart_global}.

\textbf{Theoretical Properties.}
Following \citet{casmopolitan}, we show that under typical assumptions (presented in App. \ref{app:proofs}) used for \gls{TR}-based algorithms~\citep{yuan2000review}, our proposed \ourNAS, without architecture and distillation to be introduced in §\ref{subsec:distillation}, converges to the global optimum asymptotically.
Furthermore, we derive an upper bound on the cumulative regret and show that under certain conditions it achieves sublinear regret.
We split the search space into $\mathcal{Z} = [\mathcal{H}, \mathcal{X}]$ (categorical/continuous parts respectively).
We note that \cref{assu:gp-approx} considers the minimum \gls{TR} lengths $L^x_{\min}, L^h_{\min}$ are set to be small enough so that the \gls{GP} approximates $f$ accurately in the \gls{TR}s. 
In practice, this assumption only holds asymptotically, i.e. when the observed datapoints in the \gls{TR}s goes to infinity.
We present the main result, the time-varying extension to Theorem 3.4 from \citet{casmopolitan}, and then refer to App. \ref{app:proofs} for the derivation.





\begin{theorem}
\label{thr:gconverge-mix}
Assume Assumptions \ref{assu:f-bounded} \& \ref{assu:gp-approx} hold.
Let $f_i: [\mathcal{H}, \mathcal{X}] \rightarrow \mathbb{R}$ be a time-varying objective defined over a mixed space and $\zeta \in (0, 1)$.
Suppose that:
    (i) there exists a class of functions $g_i$ in the RKHS $\mathcal{G}_k([\mathcal{H}, \mathcal{X}])$ corresponding to the kernel $k$ of the global \gls{GP} model, such that $g_i$ passes through all the local maximas of $f_i$ and shares the same global maximum as $f_i$;
    (ii) the noise at each timestep $\epsilon_i$ has mean zero conditioned on the history and is bounded by $\sigma$;
    (iii) $\Vert g_i \Vert^2_k \leq B$.
Then \ourNAS obtains a regret bound
\begin{equation} \nonumber
\text{Pr} \Big\lbrace R_{IB} \leq  \sqrt{\frac{C_1 I\beta_{I}}{B}
\gamma \bigl(IB;k;[\mathcal{H}, \mathcal{X}] \bigr)}+2 \quad \forall I \geq 1 \Big \rbrace \geq 1 - \zeta,
\end{equation}
with $C_1=8/\log(1+\sigma^{-2})$, $\gamma(T;k;[\mathcal{H}, \mathcal{X}])$ defined in \cref{thr:tv_kernel_mig} and $\beta_I$ is parameter balancing  exploration-exploitation as in Theorem 2 of \citet{pb2}.
\end{theorem}

Under the same ideal conditions assumed in~\citet{bogunovic2016time, pb2} where the objective does not vary significantly through time, the cumulative regret bound is sublinear with $\lim_{I \rightarrow \infty} \frac{R_{IB}}{I}=0$, when $\omega \rightarrow 0$ and $\tilde{N} \rightarrow I$.






\begin{figure}[t]
\vspace{-4mm}
    \begin{center}
        \includegraphics[trim=0cm 0cm 0cm  -1.1cm, clip, width=1.0\linewidth]{figures/main_fig.pdf}   
    \end{center}
    \vspace{-4mm}
        \caption{\our (a) at the \emph{beginning} of a generation (\textbf{left}) and (b) \emph{during} a generation (\textbf{right}). At the start of a generation, agents with diverse architectures are suggested and on-policy distillation is used to transfer information across generations \& different architectures (§\ref{subsec:distillation}). Within a generation, a high-dimensional, mixed-input \gls{BO} agent suggests hyperparameters (§\ref{subsec:bo}, we copy weights across fixed architectures).
        }
        \label{fig:method_picture}
        \vspace{-4mm}
\end{figure}

\subsection{Adapting Architectures on the Fly}
\label{subsec:distillation}
Now that we are equipped with an approach to optimize in high-dimensional $\mathcal{Z}$, we focus on choosing \emph{network architectures}.
Despite their importance in \gls{RL} \citep{coinrun, furuta2021pic}, architectures remain underexplored as a research direction.
Adapting architectures for \gls{PBT} methods is non-trivial as we further enlarge the search space, and weights cannot readily be copied across different networks.
Inspired by \citet{openendedlearningteam2021openended}, our key idea is that when beginning a new {\emph{generation}} we can distill behaviors into new architectures (see Fig. \ref{fig:method_picture}).
Specifically:
\begin{itemize}[noitemsep,topsep=-8pt, leftmargin=3pt]
\item
\emph{Starting each generation:} We fill the population of $B$ agents by generating a diverse set of architectures for both the policy and value networks.
For the first generation, this is done via random sampling.
For subsequent generations, we use suggestions from \gls{BO} and/or random search with successive halving over the architecture space $\mathcal{Y}$ only (refer to App. \ref{appsubsec:new_archs} for details); the \gls{BO} is trained on observations of the best performance each architecture has achieved in previous generations.
We initialize a new generation when the evaluated return stagnates beyond a pre-set patience during training.

\item
\emph{Transfer between generations:} 
Apart from the very first generation, we transfer information from the best agent(s) of the previous generation to each new agent, in a similar fashion  to~\citet{openendedlearningteam2021openended}, using on-policy distillation with a joint supervised and \gls{RL} loss between \emph{different architectures} as shown in Fig.~\ref{fig:method_picture}a.
Given a learned policy $\pi_i$ and value function $V_i$ from a previous generation, the new joint loss optimized is:
\begin{align}
\mathbb{E}_{(s_t, a_t) \sim \pi_{i+1}} [\alpha_{\mathrm{RL}}\mathcal{L}_{\mathrm{RL}} + \alpha_{V}\norm{V_i(s_t) - V_{i+1}(s_t)}_2 + \alpha_{\pi} \mathbb{D}_{\textrm{KL}}\bigl( \pi_i(\cdot \vbar s_t) \,||\, \pi_{i+1}(\cdot \vbar s_t) \bigr)]
\end{align}
for weights $\alpha_{\mathrm{RL}}\geq0$, $\alpha_{V}\geq0$, $\alpha_{\pi}\geq0$, and \gls{RL} loss $\mathcal{L}_{\mathrm{RL}}$ taken from \cref{eqn:ppo}.
We linearly anneal the supervised losses over the course of each generation, so that by the end, only the \gls{RL} loss remains.

\item
\emph{During a generation:} We follow standard \gls{PBT} methods to evolve the hyperparameters of each agent by copying weights $\btheta$ \emph{and the architecture} $\by$ from a top-$q\%$ performing agent to a bottom-$q\%$ agent, as shown in Fig.~\ref{fig:method_picture}b.
This creates an effect similar to successive halving \citep{pmlr-v28-karnin13, pmlr-v51-jamieson16} where poorly-performing architectures are quickly removed from the population in favor of more strongly-performing ones; typically at the end of a generation, 1 or 2 architectures dominate the population.
While we do not introduce new architectures within a generation, the hyperparameter suggestions are conditioned on the current policy and value architectures by incorporating the architecture parameters $\by$ as contextual fixed dimensions in the \gls{GP} surrogate described in §\ref{subsec:bo}.
\end{itemize}


==> BG-PBT (AutoML Conference)_arXiv 2/06_experiments.tex <==
\section{Experiments}
\label{sec:experiments}
While \our provides a framework applicable to any \gls{RL} algorithm, we test our method on 7 environments from the new \textsc{Brax} environment suite, using \gls{PPO}.
We begin by presenting a comparative evaluation of \our against standard baselines in population-based training to both show the benefit of searching over the full hyperparameter space with local \gls{BO} and of automatically adapting architectures over time.
We further show that our method beats end-to-end \gls{BO}, showing the advantage of dynamic schedules.
Next, we analyze these learned hyperparameter and architecture schedules using \our and we show analogies to similar trends in learning rate and batch size in supervised learning.
Finally, we perform ablations on individual components of \our.
For all population-based methods, we use a population size $B=8$ and a total budget of 150M steps.
We note that \our with architectures uses additional on-policy samples from the environment in order to distill between architectures.
We instantiate the \textsc{Brax} environments with an action repeat of 1.
We use $t_{\mathrm{ready}}$ of 1M for all \gls{PBT}-based methods on all environments except for Humanoid and Hopper, where we linearly anneal $t_{\mathrm{ready}}$ from 5M to 1M.
The remaining hyperparameters and implementation details used in this section are listed in App. \ref{app:implementation_details}.

\begin{figure}[t]
\vspace{-2mm}
\centering
     \begin{subfigure}{1\linewidth}
          \includegraphics[width=\textwidth]{figures/result_fig.pdf}
     \end{subfigure}
     \vspace{-2mm}
     \begin{subfigure}{0.4\linewidth}
       \includegraphics[width=\textwidth, trim={0, 0, 0, .6cm}, clip]{figures/combined_legend.pdf}
     \end{subfigure}
    \vspace{-3.5mm}
\caption{
    \small{Visualization of each environment (\textbf{top row}) and mean evaluated return over the population with $\pm$1 \textsc{sem} (shaded) across 7 random seeds (\textbf{bottom row}) in all environments. \texttt{RS} refers to the higher performing of RS-$\mathcal{Z}$ or RS-$\mathcal{J}$ in \cref{tab:main_results}.
    }
}
\vspace{-4mm}
\label{fig:main_fig}
\end{figure}
\begin{table}[tb]
    \centering
        \caption{{Mean evaluated return $\pm 1$\textsc{sem} across 7 seeds shown. For \gls{PBT}-style methods (\gls{PBT}, \gls{PB2} and \our), the mean best-performing agent in the population is shown. Methods performing within 1 \textsc{sem} of the best-performing method are bolded (the same applies to all tables).
        }
        }
        \vspace{-3mm}
        \begin{footnotesize}
    \adjustbox{max width=0.98\columnwidth}{
    \begin{tabular}{ccccccc}
    \toprule
     Method & \textit{PPO}$^*$ & RS & RS & PBT & PB2 & BG-PBT\\
     Search space & $\mathcal{Z}$ & $\mathcal{Z}$ & $\mathcal{J}$ & $\mathcal{Z}$ & $\mathcal{Z}$ & $\mathcal{J}$\\
    \midrule
    Ant & ${3853}_{\pm 676}$ & $6780_{\pm 317}$ & $4781_{\pm 515}$ & $8955_{\pm 385}$ &  $8954_{\pm 594}$ & $\mathbf{10349_{\pm 326}}$ \\
    HalfCheetah & ${6037}_{\pm 236}$ & $9502_{\pm 76}$ & $10340_{\pm 329}$ & $8455_{\pm 400}$ & $8629_{\pm 746}$ & $\mathbf{13450_{\pm 551}}$ \\
    Humanoid  & ${\boldsymbol{{9109}}_{\pm 987}}$ & $4004_{\pm 519}$ & $4652_{\pm 1002}$ & $7954_{\pm 437}$ & ${8452_{\pm 512}}$ & $\mathbf{9171_{\pm 748}}$ \\
    Hopper  & ${120}_{\pm 43}$ & $339_{\pm 25}$ & $943_{\pm 185}$ & $2002_{\pm 254}$ & $2027_{\pm 323}$ &  $\mathbf{2569_{\pm 293}}$\\
    Reacher & ${-189.3}_{\pm 43.7}$ & $-24.2_{\pm 1.4}$ & $-95.2_{\pm 25.3}$ & $-32.9_{\pm 2.8}$ & $-26.6_{\pm 2.6}$ & $\mathbf{{-19.2_{\pm 0.9}}}$\\
    Fetch & $\boldsymbol{{14.0}_{\pm 0.2}}$ & $5.2_{\pm 0.4}$ & $8.6_{\pm 0.2}$ & $5.5_{\pm 0.8}$ & $6.6_{\pm 0.7}$ &  ${9.4}_{\pm 0.7}$ \\    
    UR5e & ${5.2}_{\pm 0.2}$ & $5.3_{\pm 0.4}$ & $7.7_{\pm 0.3}$ & $6.9_{\pm 0.4}$ & $7.4_{\pm 0.6}$ & $\mathbf{10.7_{\pm 0.6}}$\\
    \bottomrule 
    \multicolumn{7}{l}{$^*$From the \textsc{Brax} authors and implemented in a different framework (JAX) to ours (PyTorch)}
    \end{tabular}}
    \label{tab:main_results}
    \end{footnotesize}
    \vspace{-5mm}
\end{table}

\textbf{Comparative Evaluation of \our.}
We first perform a comparative evaluation of \our against standard baselines in \gls{PBT}-methods and the \gls{PPO} baseline provided by the \textsc{Brax} authors.
We show the benefit of using local \gls{BO} and treating the whole \gls{RL} hyperparameter space $\mathcal{Z}$, by comparing \our against \gls{PBT}~\citep{PBT}, \gls{PB2}~\citep{pb2} and \gls{RS} using the default architecture in \textsc{Brax}.
In \gls{RS}, we simply sample from the hyperparameter space and take the best performance found using the same compute budget as the \gls{PBT} methods.
Next, we include architecture search into \our using the full space $\mathcal{J}$ and show significant gains in performance compared to \our without architectures; we use random search over $\mathcal{J}$ as a baseline.
The optimized \gls{PPO} implementation from the \textsc{Brax} authors is provided as a sequential baseline.
We present the results in \cref{tab:main_results} and the training trajectories in Fig.~\ref{fig:main_fig}.

We show that \our significantly outperforms the \gls{RS} baselines and the existing \gls{PBT}-style methods in almost all environments considered.
We also observe that \gls{RS} is a surprisingly strong baseline, performing on par or better than \gls{PBT} and \gls{PB2} in HalfCheetah, Reacher, Fetch and UR5e --- this is due to a well-known failure mode in \gls{PBT}-style algorithms where they may be overly greedy in copying sub-optimal behaviors early on and then fail to sufficiently explore in weight space when the population size is modest.
\our avoids this problem by \emph{re-initializing networks each generation} and distilling, which prevents collapse to suboptimal points in weight space.

\textbf{Experiments with Different Training Timescales.}
We further show experiments with a higher budget of $300$M timesteps and/or an increased population size up to $B=24$ to investigate the scalability of \our in larger-scale environments (App. \ref{app:increased_timesteps}). 
Furthermore, given that \our uses additional on-policy samples in order to distill between architectures, we conduct experiments of \our with reduced training budget in App. \ref{app:decreased_timesteps}.
We find that even when the maximum timesteps are roughly halved, \our still outperforms the baseline AutoRL methods. 

\textbf{Comparison Against Sequential \gls{BO}.} We further compare against \gls{BO} in the traditional sequential setup (Table \ref{tab:bo_comparison}): for each \gls{BO} iteration, the agent is trained for the full 150M timesteps before a new hyperparameter suggestion is made.
To enable \gls{BO} to improve on \gls{RS}, we allocate a budget of 50 evaluations, \emph{which is up to 6$\times$ more expensive} than our method and even more costly in terms of wall-clock time if vanilla, non-parallel \gls{BO} is used.
We implement this baseline using SMAC3 \citep{lindauer2022smac3} in both the $\mathcal{Z}$ and $\mathcal{J}$ search spaces (denoted BO-$\mathcal{Z}$ and BO-$\mathcal{J}$ respectively in \cref{tab:bo_comparison}).
While, unsurprisingly, \gls{BO} improves over the \gls{RS} baseline, \our still outperforms it in a majority of environments.
One reason for this is that \our naturally discovers a dynamic schedule of hyperparameters and architectures, which is strictly more flexible than a carefully tuned but still static configuration -- we analyze this below.

\begin{table}[t]
\vspace{-6mm}
\centering
\begin{minipage}{.47\linewidth}
\centering
  \captionsetup{width=.91\linewidth}
        \caption{\small{Comparison against sequential BO$^*$}
        }
        \vspace{-3mm}
        \begin{footnotesize}
    \adjustbox{max width=0.95\columnwidth}{
    \begin{tabular}{cccc}
    \toprule
     Method & BO-$\mathcal{Z}$$^*$ & BO-$\mathcal{J}$$^*$ & BG-PBT\\
    \midrule
    Ant &  $6975_{\pm 1013}$ & $7149_{\pm 507}$ & $\mathbf{10349_{\pm 326}}$ \\
    HalfCheetah & $11202_{\pm 204}$ & $10859_{\pm 174}$ &$\mathbf{13450_{\pm 551}}$ \\
    Humanoid  &  $\mathbf{9040_{\pm 1303}}$ & ${4845_{\pm 962}}$ & $\mathbf{{9171_{\pm 748}}}$ \\
    Hopper  &  $358_{\pm 60}$ & ${1254_{\pm 154}}$ &  $\mathbf{2569_{\pm 293}}$\\
    Reacher & $\mathbf{-17.3_{\pm 0.3}}$ & ${{-51.7_{\pm 18.3}}}$ &  ${{-19.2_{\pm 0.9}}}$\\
    Fetch & $\mathbf{13.2_{\pm 0.2}}$ & $11.6_{\pm 0.1}$ & ${9.4}_{\pm 0.7}$ \\    
    UR5e & $9.0_{\pm 0.5}$ & $6.3_{\pm 1.4}$ & $\mathbf{10.7_{\pm 0.6}}$\\
    \bottomrule 
    \multicolumn{4}{l}{$^*$More resources required compared to \our.}
    \end{tabular}}
    \label{tab:bo_comparison}
    \end{footnotesize}
\end{minipage}
\hfill
\begin{minipage}{.49\linewidth}
\centering
  \captionsetup{width=.95\linewidth}
        \caption{Ablation studies
        }
        \vspace{-3mm}
        \begin{footnotesize}
    \adjustbox{max width=0.95\columnwidth}{
    \begin{tabular}{cccc}
    \toprule
     Method & No TR/NAS & No NAS & BG-PBT\\
    \midrule
    Ant &  $8954_{\pm 594}$ & $9352_{\pm 402}$ & $\mathbf{10349_{\pm 326}}$ \\
    HalfCheetah & $8629_{\pm 746}$ & $9483_{\pm 626}$ &$\mathbf{13450_{\pm 551}}$ \\
    Humanoid  &  ${8452_{\pm 512}}$ & $\mathbf{10359_{\pm 647}}$ & ${9171_{\pm 748}}$ \\
    Hopper  &  $2027_{\pm 323}$ & $\mathbf{{2511_{\pm 154}}}$ &  $\mathbf{2569_{\pm 293}}$\\
    Reacher & $-26.6_{\pm 2.6}$ & $\mathbf{{-17.6_{\pm 0.8}}}$ &  ${{-19.2_{\pm 0.9}}}$\\
    Fetch & $6.6_{\pm 0.7}$ & $7.3_{\pm 0.8}$ & $\mathbf{9.4}_{\pm 0.7}$ \\    
    UR5e & $7.4_{\pm 0.6}$ & $9.0_{\pm 0.8}$ & $\mathbf{10.7_{\pm 0.6}}$\\
    \bottomrule 
    \\
    \end{tabular}}
    \label{tab:ablation}
    \end{footnotesize}
\end{minipage}
\end{table}
\begin{figure}[tb]
\vspace{-4mm}
\centering
     \centering
     \includegraphics[width=\textwidth]{figures/ant_schedule.pdf}
\vspace{-7mm}
\caption{
    \small{The hyperparameter and architecture schedule discovered by \our on Ant: we plot the hyperparameters of the best-performing agent in the population averaged across 7 seeds with $\pm$ 1 \textsc{sem} shaded. \textcolor{gray}{Gray dashed lines} denote the hyperparameter bounds.
    }
}
\vspace{-5mm}
\label{fig:ant_schedule}
\end{figure}

\textbf{Analysis of Discovered Hyperparameter and Architecture Schedules.}
We present the hyperparameter and architecture schedules learned by \our in our main comparative evaluation on Ant in Fig.~\ref{fig:ant_schedule} (results on other environments are presented in App.~\ref{app:more_schedule}).
We find consistent trends across environments such as the decrease of learning rate and increase in batch sizes over time, consistent to common practices in both \gls{RL}~\citep{Engstrom2020Implementation} and supervised learning, but crucially \our discovers the same \emph{without any pre-defined schedule}.
We note, however, that the exact rate at which the learning rate decreases and batch size increase differs across different environments -- for example, in Ant we find that the learning rate quickly drops from a relatively large value to almost the smallest possible $10^{-4}$, whereas in UR5e, the schedule is much less aggressive. This suggests that the optimal schedule is dependent on the exact environment, and a uniform, manually-defined schedule as in~\citet{Engstrom2020Implementation} may not be optimal. We demonstrate this empirically in App. \ref{app:comp_rs}, where we compare against \gls{RS} but with the learning rate following a manually-defined cosine annealing schedule.
We also find that different networks are favored at different stages of training, but the exact patterns differ across environments: for Ant (Fig.~\ref{fig:ant_schedule}), we find that larger networks are preferred towards the end of training, with the policy and value network widths increasing over time:
Prior work has shown that larger networks like those we automatically find towards the end of training \emph{can be notoriously unstable and difficult to train from scratch}~\citep{czarnecki2018mixmatch, ota2021training}, which further supports our use of generational training to facilitate this.

\textbf{Ablation Studies.}
\our improves on existing methods by using local \gls{TR}-based \gls{BO} (§\ref{subsec:bo}) and \gls{NAS} \& distillation (§\ref{subsec:distillation}).
We conduct an ablation study by removing either or both components in \cref{tab:ablation} (a comparison between the training trajectories in Fig. \ref{fig:nonas_fig} may be found in App. \ref{app:ablation}), where ``No NAS'' does not search architectures or distill but uses the default \textsc{Brax} architectures, and ``No TR/NAS'' further only uses a vanilla \gls{GP} surrogate and is identical to \gls{PB2}. 
We find the tailored \gls{BO} agent in §\ref{subsec:bo} improves performance across the board.
On the importance of \gls{NAS} \& distillation, in all environments except for Humanoid and Reacher, \our matches or outperforms ``No NAS'', despite $\mathcal{J}$ being a more complicated search space and the ``No NAS'' baseline is conditioned on strongly-performing default architectures.
We also see a particularly large gain for HalfCheetah and Fetch when we include architectures, demonstrating the effectiveness of the generational training and \gls{NAS} in our approach.
We include additional ablation studies in App. \ref{app:ablation}.











==> BG-PBT (AutoML Conference)_arXiv 2/07_conclusion.tex <==
\section{Related Work}

\textbf{On-the-fly Hyperparameter Tuning.}
Our work improves on previous \gls{PBT}~\citep{pb2, PBT, pbtbt} style methods; in particular, we build upon \citet{parkerholder2021tuning}, using a more scalable \gls{BO} step, and adding architecture search with generational learning.
\citet{fire_pbt} introduce an approach for increasing diversity in the weight space for \gls{PBT}, orthogonal to our work.
There have also been non-population-based methods for dynamic hyperparameter optimization, using bandits \citep{agent57, top, dvd, rp1,gpbo_tvo}, gradients \citep{paul2019fast, metagradients, stac, flennerhag2022bootstrapped} or Evolution \citep{online_hpo_evolutionary_arvix_20} which mostly do not search over architectures.
A notable exception is Sample-efficient Automated Deep Learning (SEARL) \citep{franke2020sample}, which adapts architectures within a \gls{PBT} framework.
However, SEARL is designed for off-policy \gls{RL} and thus especially shows the benefit of shared replay buffers for efficiency, whereas our method is general-purpose.

\textbf{Architecture Search.}
In \gls{RL}, \citet{czarnecki2018mixmatch} showed increasing agent complexity over time could be effective, albeit with a pre-defined schedule.
\citet{rl_darts} showed that DARTS \citep{liu2018darts} could be effective in \gls{RL}, finding high performing architectures on the Procgen benchmark.
Auto-Agent-Distiller~\citep{fu2020autoagentdistiller} deals with the problem of finding optimal architectures for compressing the model size of \gls{RL} agents, and also find that using distillation between the teacher and student networks improves stability of \gls{NAS} in \gls{RL}.
On the other hand, \gls{BO} has been used as a powerful tool for searching over large architecture spaces~\citep{casmopolitan, kandasamy2018neural, ru2020interpretable, white2019bananas,nguyen2021optimal, wan2022approximate}.
Conversely, we only consider simple \gls{MLP}s and the use of spectral normalization.
There has been initial effort~\citep{izquierdo2021bag} combining \gls{NAS} and hyperparameter optimization in sequential settings, which is distinct to our on-the-fly approach.

\textbf{Generational Training and Distillation.}
\cite{openendedlearningteam2021openended} recently introduced generational training, using policy distillation to transfer knowledge between generations, accelerating training.
Our method is based on this idea, with changing generations.
The use of distillation is further supported by \citet{igl2021transient} who recently used this successfully to adapt to non-stationarities in reinforcement learning, however keeping hyperparameters and architectures fixed.

\section{Conclusion \& Discussion}
\label{sec:conclusion}
In this paper, we propose \our: a new algorithm that significantly increases the capabilities of \gls{PBT} methods for \gls{RL}.
Using recent advances in Bayesian Optimization, \our is capable of searching over drastically larger search spaces than previous methods.
Furthermore, inspired by recent advances in generational learning, we show it is also possible to efficiently learn architectures on the fly as part of a unified algorithm.
The resulting method leads to significant performance gains across the entire  \textsc{Brax} environment suite, achieving high performance even in previously untested environments.
We believe \our is a significant step towards truly environment agnostic RL algorithms, while also offering a path towards open-ended learning where agents never stop tuning themselves and continuously expand their capabilities over time. 


==> BG-PBT (AutoML Conference)_arXiv 2/08_limitations.tex <==

\textbf{Limitations \& Future Work.}
We note that while our method shows a significant boost in performance by including architectures for most environments, in some environments, such as Humanoid, we achieve better results without architecture search (Table \ref{tab:ablation}).
We hypothesize this is due to the complexity of the environment and an increased sensitivity to the network architecture.
Furthermore, while we provide a theoretical guarantee for our method in \cref{thr:gconverge-mix} for searching purely over architectures, no such guarantees exist when we transfer between architectures across generations.
Indeed, we occasionally see poor architectures being selected, which are then discarded during truncation selection.
Therefore, an immediate future direction is to address these issues and to improve the architecture selection process.
Another limitation is that while all \gls{RL}-related hyperparameters are included in the search space, certain hyperparameters of \our could also be automatically searched for, including but not limited to distillation hyperparameters, which are currently fixed, and \gls{PBT} parameters such as $t_{\mathrm{ready}}$, which could allow us to avoid myopic and greedy behavior.
Beyond these limitations, our algorithm readily transfers to other \gls{RL} problems with high-dimensional mixed spaces, and thus we would readily accommodate more complicated architecture search spaces (e.g. vision-based environments) and incorporate environment parameters~\citep{DBLP:journals/corr/PaulCOW16} into the search space to generalize to new tasks.

\textbf{Broader Impact.}
We open-source our code so that practitioners in the field can accelerate their own deployment of \gls{RL} systems.
However, in doing so, we should be wary of the risk of also improving malicious use of \gls{RL}; in particular, down-stream applications which could have an impact on people's security and privacy.
To mitigate these risks, we encourage research on \gls{RL} governance and safe \gls{RL}.
As a general purpose framework for improving any \gls{RL} algorithm, our method should be part of that conversation.

==> BG-PBT (AutoML Conference)_arXiv 2/09_reproducibility.tex <==
\clearpage
\section{Reproducibility Checklist}


\begin{enumerate}
\item For all authors\dots
  \begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately
    reflect the paper's contributions and scope?
    \answerYes{[The abstract and introduction's content is substantiated in §\ref{sec:experiments}]}
  \item Did you describe the limitations of your work?
    \answerYes{We discuss them in §\ref{sec:conclusion}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{We discuss them in §\ref{sec:conclusion}.}
  \item Have you read the ethics review guidelines and ensured that your paper
    conforms to them?
    \answerYes{We have ensured our paper conforms to the guidelines.}
  \end{enumerate}
\item If you are including theoretical results\dots
  \begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{The full set of assumptions are provided in \cref{app:proofs}.}
  \item Did you include complete proofs of all theoretical results?
    \answerYes{Complete proofs provided in \cref{app:proofs}.}
  \end{enumerate}
\item If you ran experiments\dots
  \begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the
    main experimental results, including all requirements (e.g.,
    \texttt{requirements.txt} with explicit version), an instructive
    \texttt{README} with installation, and execution commands (either in the
    supplemental material or as a \textsc{url})?
    \answerYes{We have included this in the supplementary material.}
  \item Did you include the raw results of running the given instructions on the
    given code and data?
    \answerYes{We include raw numbers produced by the code.}
  \item Did you include scripts and commands that can be used to generate the
    figures and tables in your paper based on the raw results of the code, data,
    and instructions given?
    \answerYes{We include notebooks that produce the plots.}
  \item Did you ensure sufficient code quality such that your code can be safely
    executed and the code is properly documented?
    \answerYes{Yes, the code is documented and appropriate commands provided.}
  \item Did you specify all the training details (e.g., data splits,
    pre-processing, search spaces, fixed hyperparameter settings, and how they
    were chosen)?
    \answerYes{Implementation details are discussed in \cref{app:full_search_space} and \cref{app:implementation_details}.}
  \item Did you ensure that you compared different methods (including your own)
    exactly on the same benchmarks, including the same datasets, search space,
    code for training and hyperparameters for that code?
    \answerYes{All methods benchmarked on the same \textsc{Brax} environment suite, we used the same computational budget and population size for all other PBT methods.}
  \item Did you run ablation studies to assess the impact of different
    components of your approach?
    \answerYes{We include ablations in \cref{sec:experiments} and in \cref{app:additional_experiments}.}
  \item Did you use the same evaluation protocol for the methods being compared?
    \answerYes{All PBT methods are evaluated by best performance in the population.}
  \item Did you compare performance over time?
    \answerYes{We regularly evaluate the evaluated performance through the course of training.}
  \item Did you perform multiple runs of your experiments and report random seeds?
    \answerYes{All our experiments are averaged over 7 random seeds.}
  \item Did you report error bars (e.g., with respect to the random seed after
    running experiments multiple times)?
    \answerYes{We report the mean performance and indicate $\pm$ 1 standard error.}
  \item Did you use tabular or surrogate benchmarks for in-depth evaluations?
    \answerNA{}{}
  \item Did you include the total amount of compute and the type of resources
    used (e.g., type of \textsc{gpu}s, internal cluster, or cloud provider)?
    \answerYes{We describe our compute and resource usage in \cref{app:implementation_details}.}
  \item Did you report how you tuned hyperparameters, and what time and
    resources this required (if they were not automatically tuned by your AutoML method, e.g. in a \textsc{nas} approach; and also hyperparameters of your
    own method)?
    \answerYes{The RL hyperparameters were tuned by our AutoRL method. The hyperparameters for \our were tuned by hand with ablations performed in \cref{app:additional_experiments}.}
  \end{enumerate}
\item If you are using existing assets (e.g., code, data, models) or
  curating/releasing new assets\dots
  \begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We cite the creators of the codebase we use in \cref{app:implementation_details}.}
  \item Did you mention the license of the assets?
    \answerYes{We mention the license of the codebase we use in \cref{app:implementation_details}.}
  \item Did you include any new assets either in the supplemental material or as a \textsc{url}?
    \answerYes{We include figures in a url link in the introduction.}
  \item Did you discuss whether and how consent was obtained from people whose
    data you're using/curating?
    \answerNA{No personal data used. All data for our algorithm is generated from RL environments.}
  \item Did you discuss whether the data you are using/curating contains
    personally identifiable information or offensive content?
    \answerNA{No personal data used. All data for our algorithm is generated from RL environments.}
  \end{enumerate}
\item If you used crowdsourcing or conducted research with human subjects\dots
  \begin{enumerate}
  \item Did you include the full text of instructions given to participants and
    screenshots, if applicable?
    \answerNA{[We are not crowdsourcing or conducting research with human subjects.]}
  \item Did you describe any potential participant risks, with links to
    Institutional Review Board (\textsc{irb}) approvals, if applicable?
    \answerNA{[We are not crowdsourcing or conducting research with human subjects.]}
  \item Did you include the estimated hourly wage paid to participants and the
    total amount spent on participant compensation?
    \answerNA{[We are not crowdsourcing or conducting research with human subjects.]}
  \end{enumerate}
\end{enumerate}

==> BG-PBT (AutoML Conference)_arXiv 2/10_ack.tex <==
\begin{acknowledgements}
XW and BR are supported by the Clarendon Scholarship at the University of Oxford.
CL is funded by the Engineering and Physical Sciences Research Council (EPSRC). 
PB is funded through the Willowgrove Studentship.
The authors would like to thank Yee Whye Teh for detailed feedback on an early draft and the anonymous AutoML conference reviewers \& the area chair for their constructive comments which helped improve the paper.
\end{acknowledgements}


==> BG-PBT (AutoML Conference)_arXiv 2/macros.tex <==
\global\long\def\se{\hat{\text{se}}}%

\global\long\def\interior{\text{int}}%

\global\long\def\boundary{\text{bd}}%

\global\long\def\new{\text{*}}%

\global\long\def\stir{\text{Stirl}}%

\global\long\def\dist{d}%

\global\long\def\HX{\entro\left(X\right)}%
 
\global\long\def\entropyX{\HX}%

\global\long\def\HY{\entro\left(Y\right)}%
 
\global\long\def\entropyY{\HY}%

\global\long\def\HXY{\entro\left(X,Y\right)}%
 
\global\long\def\entropyXY{\HXY}%

\global\long\def\mutualXY{\mutual\left(X;Y\right)}%
 
\global\long\def\mutinfoXY{\mutualXY}%

\global\long\def\xnew{y}%

\global\long\def\bx{\mathbf{x}}%

\global\long\def\bh{\mathbf{h}}%

\global\long\def\bw{\mathbf{w}}%

\global\long\def\bz{\mathbf{z}}%

\global\long\def\bu{\mathbf{u}}%

\global\long\def\bs{\boldsymbol{s}}%

\global\long\def\bk{\mathbf{k}}%

\global\long\def\bX{\mathbf{X}}%

\global\long\def\tbx{\tilde{\bx}}%

\global\long\def\by{\mathbf{y}}%

\global\long\def\bY{\mathbf{Y}}%

\global\long\def\bZ{\boldsymbol{Z}}%

\global\long\def\bU{\boldsymbol{U}}%

\global\long\def\bv{\boldsymbol{v}}%

\global\long\def\balpha{\boldsymbol{\alpha}}

\global\long\def\btheta{\boldsymbol{\theta}}

\global\long\def\bn{\boldsymbol{n}}%

\global\long\def\bV{\boldsymbol{V}}%

\global\long\def\bK{\boldsymbol{K}}%

\global\long\def\bbeta{\gvt{\beta}}%

\global\long\def\bmu{\gvt{\mu}}%

\global\long\def\btheta{\boldsymbol{\theta}}%

\global\long\def\blambda{\boldsymbol{\lambda}}%

\global\long\def\bgamma{\boldsymbol{\gamma}}%

\global\long\def\bpsi{\boldsymbol{\psi}}%

\global\long\def\bphi{\boldsymbol{\phi}}%

\global\long\def\bpi{\boldsymbol{\pi}}%

\global\long\def\eeta{\boldsymbol{\eta}}%

\global\long\def\bomega{\boldsymbol{\omega}}%

\global\long\def\bepsilon{\boldsymbol{\epsilon}}%

\global\long\def\btau{\boldsymbol{\tau}}%

\global\long\def\bSigma{\gvt{\Sigma}}%

\global\long\def\realset{\mathbb{R}}%

\global\long\def\realn{\realset^{n}}%

\global\long\def\integerset{\mathbb{Z}}%

\global\long\def\natset{\integerset}%

\global\long\def\integer{\integerset}%
 

\global\long\def\natn{\natset^{n}}%

\global\long\def\rational{\mathbb{Q}}%

\global\long\def\rationaln{\rational^{n}}%

\global\long\def\complexset{\mathbb{C}}%

\global\long\def\comp{\complexset}%
 

\global\long\def\compl#1{#1^{\text{c}}}%

\global\long\def\and{\cap}%

\global\long\def\compn{\comp^{n}}%

\global\long\def\comb#1#2{\left({#1\atop #2}\right) }%

\global\long\def\nchoosek#1#2{\left({#1\atop #2}\right)}%

\global\long\def\param{\vt w}%

\global\long\def\Param{\Theta}%

\global\long\def\meanparam{\gvt{\mu}}%

\global\long\def\Meanparam{\mathcal{M}}%

\global\long\def\meanmap{\mathbf{m}}%

\global\long\def\logpart{A}%

\global\long\def\simplex{\Delta}%

\global\long\def\simplexn{\simplex^{n}}%

\global\long\def\dirproc{\text{DP}}%

\global\long\def\ggproc{\text{GG}}%

\global\long\def\DP{\text{DP}}%

\global\long\def\ndp{\text{nDP}}%

\global\long\def\hdp{\text{HDP}}%

\global\long\def\gempdf{\text{GEM}}%

\global\long\def\ei{\text{EI}}%

\global\long\def\rfs{\text{RFS}}%

\global\long\def\bernrfs{\text{BernoulliRFS}}%

\global\long\def\poissrfs{\text{PoissonRFS}}%

\global\long\def\grad{\gradient}%
 
\global\long\def\gradient{\nabla}%

\global\long\def\cpr#1#2{\Pr\left(#1\ |\ #2\right)}%

\global\long\def\var{\text{Var}}%

\global\long\def\Var#1{\text{Var}\left[#1\right]}%

\global\long\def\cov{\text{Cov}}%

\global\long\def\Cov#1{\cov\left[ #1 \right]}%

\global\long\def\COV#1#2{\underset{#2}{\cov}\left[ #1 \right]}%

\global\long\def\corr{\text{Corr}}%

\global\long\def\sst{\text{T}}%

\global\long\def\SST{\sst}%

\global\long\def\ess{\mathbb{E}}%
 

\global\long\def\Ess#1{\ess\left[#1\right]}%


\global\long\def\fisher{\mathcal{F}}%
 

\global\long\def\bfield{\mathcal{B}}%
 
\global\long\def\borel{\mathcal{B}}%

\global\long\def\bernpdf{\text{Bernoulli}}%

\global\long\def\betapdf{\text{Beta}}%

\global\long\def\dirpdf{\text{Dir}}%

\global\long\def\gammapdf{\text{Gamma}}%

\global\long\def\gaussden#1#2{\text{Normal}\left(#1, #2 \right) }%

\global\long\def\gauss{\mathbf{N}}%

\global\long\def\gausspdf#1#2#3{\text{Normal}\left( #1 \lcabra{#2, #3}\right) }%

\global\long\def\multpdf{\text{Mult}}%

\global\long\def\poiss{\text{Pois}}%

\global\long\def\poissonpdf{\text{Poisson}}%

\global\long\def\pgpdf{\text{PG}}%

\global\long\def\wshpdf{\text{Wish}}%

\global\long\def\iwshpdf{\text{InvWish}}%

\global\long\def\nwpdf{\text{NW}}%

\global\long\def\niwpdf{\text{NIW}}%

\global\long\def\studentpdf{\text{Student}}%

\global\long\def\unipdf{\text{Uni}}%

\global\long\def\transp#1{\transpose{#1}}%
 
\global\long\def\transpose#1{#1^{\mathsf{T}}}%

\global\long\def\mgt{\succ}%

\global\long\def\mge{\succeq}%

\global\long\def\idenmat{\mathbf{I}}%

\global\long\def\trace{\mathrm{tr}}%

\global\long\def\argmax#1{\underset{_{#1}}{\text{argmax}} }%

\global\long\def\argmin#1{\underset{_{#1}}{\text{argmin}\ } }%

\global\long\def\diag{\text{diag}}%

\global\long\def\norm{}%

\global\long\def\spn{\text{span}}%

\global\long\def\vtspace{\mathcal{V}}%

\global\long\def\field{\mathcal{F}}%
 
\global\long\def\ffield{\mathcal{F}}%

\global\long\def\inner#1#2{\left\langle #1,#2\right\rangle }%
 
\global\long\def\iprod#1#2{\inner{#1}{#2}}%

\global\long\def\dprod#1#2{#1 \cdot#2}%

\global\long\def\norm#1{\left\Vert #1\right\Vert }%

\global\long\def\entro{\mathbb{H}}%

\global\long\def\entropy{\mathbb{H}}%

\global\long\def\Entro#1{\entro\left[#1\right]}%

\global\long\def\Entropy#1{\Entro{#1}}%

\global\long\def\mutinfo{\mathbb{I}}%

\global\long\def\relH{\mathit{D}}%

\global\long\def\reldiv#1#2{\relH\left(#1||#2\right)}%

\global\long\def\KL{KL}%

\global\long\def\KLdiv#1#2{\KL\left(#1\parallel#2\right)}%
 
\global\long\def\KLdivergence#1#2{\KL\left(#1\ \parallel\ #2\right)}%

\global\long\def\crossH{\mathcal{C}}%
 
\global\long\def\crossentropy{\mathcal{C}}%

\global\long\def\crossHxy#1#2{\crossentropy\left(#1\parallel#2\right)}%

\global\long\def\breg{\text{BD}}%

\global\long\def\lcabra#1{\left|#1\right.}%

\global\long\def\lbra#1{\lcabra{#1}}%

\global\long\def\rcabra#1{\left.#1\right|}%

\global\long\def\rbra#1{\rcabra{#1}}%


